LLM-as-BT-Planner: Leveraging LLMs for Behavior Tree Generation in Robot Task Planning

Robotic assembly tasks remain an open challenge due to their long horizon nature and complex part relations. Behavior trees (BTs) are increasingly used in robot task planning for their modularity and flexibility, but creating them manually can be effort-intensive. Large language models (LLMs) have recently been applied to robotic task planning for generating action sequences, yet their ability to generate BTs has not been fully investigated. To this end, we propose LLM-as-BT-Planner, a novel framework that leverages LLMs for BT generation in robotic assembly task planning. Four in-context learning methods are introduced to utilize the natural language processing and inference capabilities of LLMs for producing task plans in BT format, reducing manual effort while ensuring robustness and comprehensibility. Additionally, we evaluate the performance of fine-tuned smaller LLMs on the same tasks. Experiments in both simulated and real-world settings demonstrate that our framework enhances LLMs' ability to generate BTs, improving success rate through in-context learning and supervised fine-tuning.

==> header_image.tex <==

\begin{figure*}[ht]
\centering
\vspace{-20pt}
\includegraphics[width=0.85\linewidth]{pic/new/corl_headline_comb.drawio-com.png}
\caption{
% \textbf{LLM as BT-planner}
Our framework
leverages LLMs to generate executable BTs directly based on scene states and user instructions. \textbf{Left}: The conceptual overview of the framework. The LLM takes user instructions as input, generating BT-based task plans based on the scene information and the task knowledge. Unlike pick-and-place tasks that only require simple robot-object interaction, the assembly tasks require the robot to select appropriate tools to manipulate and assemble the parts. \textbf{Right}: The framework's workflow, including high-level assembly task decomposition, 
mid-level behavior tree planning, 
and low-level action execution. 
The red dashed rectangular indicates the part that our proposed methods can substitute.
} \label{fig:headline}
\vspace{-17pt}
\end{figure*}

